Robust Online Monitoring of Signal Temporal Logic

Signal Temporal Logic (STL) is a formalism used to rigorously specify requirements of cyberphysical systems (CPS), i.e., systems mixing digital or discrete components in interaction with a continuous environment or analog com- ponents. STL is naturally equipped with a quantitative semantics which can be used for various purposes: from assessing the robustness of a specification to guiding searches over the input and parameter space with the goal of falsifying the given property over system behaviors. Algorithms have been proposed and implemented for offline computation of such quantitative semantics, but only few methods exist for an online setting, where one would want to monitor the satisfaction of a formula during simulation. In this paper, we formalize a semantics for robust online monitoring of partial traces, i.e., traces for which there might not be enough data to decide the Boolean satisfaction (and to compute its quantitative counterpart). We propose an efficient algorithm to compute it and demonstrate its usage on two large scale real-world case studies coming from the automotive domain and from CPS education in a Massively Open Online Course (MOOC) setting. We show that savings in computationally expensive simulations far outweigh any overheads incurred by an online approach.

==> diesel_engine_study.tex <==

Here, we consider an industrial model of a prototype airpath system in a diesel
engine implemented in Simulink\rt. The closed-loop model consists of a plant
model describing the airpath dynamics, and a controller implementing a
proprietary control scheme.  The model has more than $3000$ blocks, with more
than $20$ lookup tables that approximate high-dimensional nonlinear functions.
Due to the significant model complexity, the speed of simulation in Simulink\rt
is about $5$ times slower, \ie, simulating $1$ second of operation takes $5$
seconds in Simulink\rt.  It is important to simulate this model over a long
time-horizon, in order to characterize the airpath behavior over extended
periods of time. Thus, savings in simulation-time by early detection of
requirement violations is very beneficial in this setup.  We choose two
parameterized safety requirements for the closed-loop design after discussions
with the control designers, as shown in
Eq.~\eqref{eq:diesel_prop1}-\eqref{eq:diesel_prop2}. Due to proprietary
concerns, we suppress the actual values of the parameters used in the
requirements.
\vspace{-0.5em}
\begin{eqnarray}
\fover(\mathbf{p_1})\!\! &\!\! = \!\! & \alw_{[a,b]}(\vx < c) 
    \label{eq:diesel_prop1} \\
\ftemp(\mathbf{p_2})\!\! &\!\! = \!\! & \alw_{[a,b]}(\abs{\vx} > c\! \implies\!\!(\ev_{[0, d]}\!\abs{\vx} < e ))
    \label{eq:diesel_prop2}
\end{eqnarray}

Property $\fover$ with parameters $\mathbf{p_1} = (a,b,c)$ specifies
that in the interval $[a,b]$, the overshoot on the signal $\vx$ should
remain below a certain threshold $c$.  Property $\ftemp$ with
parameters $\mathbf{p_2} = (a,b,c,d,e)$ is a specification on the
settling time of the signal $\vx$.  It specifies that in the time
interval $[a,b]$ if at some time $t$, $\abs{\vx}$ exceeds $c$ then it
settles to a small region ($\abs{\vx} < e$) before $t+d$.  In
\tabref{diesel}, we consider three different valuations $\nu_1$,
$\nu_2$, $\nu_3$ for $\mathbf{p_1}$ in the requirement
$\fover(\mathbf{p_1})$, and two different valuations $\nu_4$, $\nu_5$
for $\mathbf{p_2}$ in the requirement $\ftemp(\mathbf{p_2})$.

The main reason for the better performance of the online algorithm is
that simulations are time-consuming for this model.  The online
algorithm can terminate a simulation earlier (either because it
detected a violation or obtained a concrete robust satisfaction
interval), thus obtaining significant savings.  For $\fover(\nu_3)$,
we choose the parameter values for $a$ and $b$ such that the online
algorithm has to process the entire signal trace, and is thus unable
to terminate earlier.  Here we see that the total overhead (in terms
of runtime) incurred by the extra book-keeping that the online
algorithm performs is negligible (about $0.1$\%).

\begin{table}[t]
\centering
\begin{tabular}{l cc cc}
\toprule
Requirement     & \#Tr  & \#ET & \mtc{Sim. Time (hours)} \\
\cline{4-5}
                &        &     & Offline  & Online        \\
\midrule          
$\fover(\nu_1)$ & 1000   & 801  & 33.3803  & 26.1643      \\
$\fover(\nu_2)$ & 1000   & 239  & 33.3805  & 30.5923      \\
$\fover(\nu_3)$ & 1000   & 0    & 33.3808  & 33.4369      \\
$\ftemp(\nu_4)$ & 1000   & 595  & 33.3822  & 27.0405      \\
$\ftemp(\nu_5)$ & 1000   & 417  & 33.3823  & 30.6134      \\
\bottomrule
\end{tabular}

\caption{Experimental results on DEM.}
\label{tab:diesel}
\end{table}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> environments.tex <==
% \newcounter{rmrk}
% \newcounter{def}
% \newcounter{exa}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{claim}[theorem]{Claim}
% \newtheorem{problem}[theorem]{Problem}
% \newtheorem{remark}[rmrk]{Remark}
% \let\oldremark\remark
% \renewcommand{\remark}{\oldremark\normalfont}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{construction}[theorem]{Construction}
% \newtheorem{definition}[def]{Definition}
% \newtheorem{example}[exa]{Example}
% \newtheorem{proof}[theorem]{Proof}


==> mooc_study.tex <==
CPSGrader~\cite{juniwal-emsoft14,cpsgrader-www} is a publicly-available
automatic grading and feedback generation tool for online virtual labs in
cyber-physical systems.  It employs temporal logic based testers to check for
common fault patterns in student solutions for lab assignments. CPSGrader uses
the National Instruments Robotics Environment Simulator to generate traces from
student solutions and monitors STL properties (each corresponding to a
particular faulty behavior) on them. In the published version of
CPSGrader~\cite{juniwal-emsoft14}, this is done in an offline fashion by first
running the complete simulation until a pre-defined cut-off and then monitoring
the STL properties on offline traces. At a step-size of 5 ms, simulating 6
sec. of real-world operation of the system takes 1 sec. for the simulator.
When students use CPSGrader for active feedback generation and debugging,
simulation constitutes the major chunk of the application response time. Online
monitoring helps in reducing the response time by avoiding unnecessary
simulation, giving the student feedback as soon as the faulty behavior is
detected.

In order to evaluate our online monitoring algorithm, we obtained the traces and STL properties used
in the published version of CPSGrader~\cite{juniwal-emsoft14,cpsgrader-www}. These traces are the
result of running actual student submissions on a battery of tests. For lack of space, we refer the
reader to~\cite{juniwal-emsoft14} for details about the tests and STL properties. As an illustrative
example, we show the ``$\tbKB$'' property in Eq.~\ref{eq:keep_bump}: \vspace{-0.5em}
\begin{eqnarray}
    \fkb &=& \ev_{[0, 60]} \alw_{[0, 5]} \fbump
    \label{eq:keep_bump}\\
    \fbump &=& \bumpr(t) \lor \bumpl(t)
\end{eqnarray}

For each STL property, Table~\ref{tab:mooc_study} compares the total simulation
time needed for both the online and offline approaches, summed over all traces.
For the offline approach, a suitable simulation cut-off time of 60 sec is chosen
taking into account the horizons of the formulae. At a step-size of 5 ms, each
trace is roughly of length 1000. For the online algorithm, simulation terminates
before this cut-off if the truth value of the property becomes known, otherwise
it terminates at the cut-off. Table~\ref{tab:mooc_study} also shows the
monitoring overhead incurred by a na\"{i}ve online algorithm that performs
complete recomputation at every step against the overhead incurred by
Alg.~\ref{algo:online_monitoring}.

\begin{table}[t]
    \setlength{\tabcolsep}{2pt}
\centering
\footnotesize{%
    \begin{tabular}{@{\extracolsep{\fill}}l cc cc c rr}
\toprule
\multicolumn{1}{L{1.5cm}}{STL Test Bench} &  \multicolumn{1}{C{0.8cm}}{\#Tr} &
\multicolumn{1}{C{0.8cm}}{\#ET} & 
% \multicolumn{2}{C{2.4cm}}{Simulation Time (mins)} &
\multicolumn{2}{c}{Sim. Time (mins)} &
\multicolumn{1}{C{0.25cm}}{}&
% \multicolumn{2}{C{2.2cm}}{Overhead (secs)}\\
\multicolumn{2}{c}{Overhead (secs)}\\
\cline{4-5} \cline{7-8}
% {}  &  {}  &  {}  & \textit{Offline} & \textit{Online} & \textit{Na\"{i}ve} & \textit{Alg.~\ref{algo:online_monitoring}} \\
{}  &  {}  &  {}  & Offline & Online && Na\"{i}ve & Alg.~\ref{algo:online_monitoring} \\
\midrule
$\tbAF$ & 1776 & 466 & 296 & 258 &&  553 &  9 \\
$\tbAL$ & 1778 & 471 & 296 & 246 && 1347 & 30 \\
$\tbAR$ & 1778 & 583 & 296 & 226 && 1355 & 30 \\
$\tbHCa$& 1777 &  19 & 395 & 394 &&  919 & 11 \\
$\tbHCb$& 1556 & 176 & 259 & 238 &&  423 &  7 \\
$\tbHCc$& 1556 & 124 & 259 & 248 &&  397 &  7 \\
$\tbF$  & 1451 &  78 & 242 & 236 &&  336 &  6 \\
$\tbKB$ & 1775 & 468 & 296 & 240 && 1.2e4 & 268 \\
$\tbWH$ & 1556 &  71 & 259 & 253 && 1.9e4 & 1.5e3 \\
\bottomrule
\end{tabular}
}

\caption{\small{Evaluation of online monitoring for CPSGrader. Each STL Test
        Bench has an associated STL property. 
}}

\label{tab:mooc_study}
\end{table}

Table~\ref{tab:mooc_study} demonstrates that online monitoring ends up
saving up to 24\% simulation time ($>10$\% in a majority of cases.) The
monitoring overhead of Alg.~\ref{algo:online_monitoring} is negligible ($<1$\%)
as compared to the simulation time and it is less than the overhead of
the na\"{i}ve online approach consistently by a factor of 40x to 80x.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> proof1.tex <==
\begin{figure}[h!]
\centering
\begin{tikzpicture}

\node[circle,fill=black,minimum width=2mm,inner sep=0pt,
      label=above:{$t-d$}] (td) {};
\node[circle,fill=black,minimum width=2mm,inner sep=0pt,right
      of=td,label=above:{$t$},node distance=25mm] (t) {};
\node[circle,fill=black,minimum width=2mm,inner sep=0pt,right
      of=t,label=above:{$\newTime-d$},node distance=10mm] (tdp) {};
\node[circle,fill=black,minimum width=2mm,inner sep=0pt,right
      of=tdp,label=above:{$\newTime$},node distance=25mm] (tp) {};

\draw (td) to (t);
\draw[dashed] (t) to (tdp);
\draw[dashed] (tdp) to (tp);

\node[circle,fill=black,minimum width=2mm,inner sep=0pt,
      label=above:{$t-d$},below of=td,node distance=12mm] (td2) {};
\node[circle,fill=black,minimum width=2mm,inner sep=0pt,right
      of=td2,label=above:{$t$},node distance=25mm] (t2) {};
\node[circle,fill=black,minimum width=2mm,inner sep=0pt,left
      of=t2,label=above:{$\newTime-d$},node distance=10mm] (tdp2) {};
\node[circle,fill=black,minimum width=2mm,inner sep=0pt,right
      of=tdp2,label=above:{$\newTime$},node distance=25mm] (tp2) {};

\draw (td2) to (t2);
\draw[dashed] (t2) to (tp2);

\end{tikzpicture}



\caption{Two cases for where new value $\newValue$ can
occur.\label{fig:proof1}}

\end{figure}


==> untimed.tex <==
\newcommand{\sub}{\mathsf{sub}}
\newcommand{\WL}[1]{\mathsf{W}(#1)}
\newcommand{\psione}{\varphi}
\newcommand{\psitwo}{\psi}
\newcommand{\WLone}[1]{\mathsf{W_\psione}(#1)}
\newcommand{\WLtwo}[1]{\mathsf{W_\psitwo}(#1)}


If the STL formula being monitored has untimed (\ie infinite-horizon)
temporal operators, a direct application of
Alg.~\ref{algo:online_monitoring} requires every node in the sub-tree
rooted at the untimed operator to have a time horizon that is
unbounded, or in other words, the algorithm would have to keep track
of every value over arbitrarily long intervals.  For a large class of
formulae (shown in Theorem~\ref{thm:finiteness}), we can can perform
robust online monitoring using only a constant amount of memory.  The
question whether an arbitrary STL formula outside of the fragment
stated thus far can be monitored using constant memory remains an open
problem.  We now show how constant memory monitoring can be performed
for the first set of formulae. In what follows, we assume that the
subformulae $\varphi$ and $\psi$ are atomic predicates of the form
$f(\vx) > 0$. 

First, we introduce some equivalences over intervals $a,b,c$ that we use in
the theorem and the proof to follow:
\begin{eqnarray}
\min(\max(a,b),\max(a,c)) & = & \max(a, \min(b,c))           \label{eq:equivone} \\
\min(a,\max(b,c))         & = & \max( \min(a,b), \min(a,c) ) \label{eq:equivtwo} \\
\max(\max(a,b), c)        & = & \max(a,b,c)                  \label{eq:equivthree} \\
\min(\max(a,b),a)         & = & a                            \label{eq:equivfour}
\end{eqnarray}

\begin{theorem}
\label{thm:finiteness}
For each of the following formulae, where $\varphi$ and $\psi$ are atomic
predicates of the form $f(\vx)\!>\!0$, we can monitor interval robustness in an
online fashion using constant memory: (1) $\alw \varphi$, $\ev \varphi$,
(2) $\varphi \Until \psi$, (3) $\alw(\varphi \vee \ev \psi)$, $\ev(\varphi \wedge
\alw \psi)$, (4) $\alw \ev \varphi$, $\ev \alw \varphi$, and (5)
$\ev(\varphi \wedge \ev \psi)$, $\alw(\varphi \vee \alw \psi)$.
\end{theorem}

\begin{proof} 
In what follows, we use the following short-hand notation:
\begin{equation}
\label{eq:pq}
\begin{array}{lll@{\hspace{2em}}lll}
p_i & \equiv & \introb(f(\vx)\!>\!0, \pvx{n+1},t_i) &
q_i & \equiv & \introb(g(\vx)\!>\!0, \pvx{n+1},t_i) 
\end{array}
\end{equation}
\noindent Note that if $i \in [0,n]$, then $p_i$ is the same over the
partial signal $\pvx{n}$, \ie, $p_i = \introb(f(\vx)\!>\!0, \pvx{n},
t_i)$ (and respectively for $q_i$). We will use this equivalence in
several of the steps in what follows.

\noindent \textbf{(1)} $\alw \varphi$, where $\varphi \equiv f(\vx) > 0$. Observe the following:
\begin{equation}
\begin{array}{ll}
\introb(\varphi, \pvx{n+1}, 0) 
& = \dmin_{i \in [0,n+1]} p_i 
 = \dmin \left( \dmin_{i \in [0,n]} p_i,\  p_{n+1} \right) 
\end{array}
\end{equation}
In the final expression above, observe that the first entry does not
contain any $p_{n+1}$ terms, \ie, it can be computed using the data
points $\vx_1, \ldots, \vx_n$ in the partial signal $\pvx{n}$ itself.
Thus, for all $n$, if we maintain the one interval representing the
$\dmin$ of the first $n$ values of $f(\vx)$ as a {\em summary}, then
we can compute the interval robustness of $\alw(f(\vx)\!>\!0)$ over
$\pvx{n+1}$ with the additional data $\vx_{n+1}$ available at
$t_{n+1}$. Note for the dual formula $\ev(f(\vx)\!>\!0)$, a similar
result holds with $\dmin$ substituted by $\dmax$.

\noindent \textbf{(2)} $\varphi \Until \psi$, 
where $\varphi \equiv
f(\vx)\!>\!0$, and $\psi \equiv g(\vx)\!>\!0$. 
Observe the following:
\begin{equation}
\label{eq:until_introb}
\introb(\varphi \Until \psi, \pvx{n+1}, 0)  = \dmax_{i \in [0,n+1]} \dmin(q_i, \dmin_{j\in[0,i]} p_j)
\end{equation}
\noindent We can rewrite the RHS of Eq.~\eqref{eq:until_introb} to get:
\begin{equation}
\dmax\left( \underline{\dmax_{i\in[0,n]} \dmin\left(q_i, \dmin_{j\in[0,i]} p_j\right)},\quad
          \dmin\left( \underline{\dmin_{j\in[0,n]} p_j},\ p_{n+1}, q_{n+1} \right) \right) 
\end{equation}
\noindent Let $U_n$ and $M_n$ respectively denote the first and second
underlined terms in the above expression.  Note that for any $n$,
$U_n$ and $M_n$ can be computed only using data $\vx_1,\ldots,\vx_n$.
Consider the recurrences $M_{n+1} = \dmin(M_n, p_{n+1}, q_{n+1})$ and
$U_{n+1} = \dmax(U_n, M_{n+1})$; we can observe that to compute
$M_{n+1}$ and $U_{n+1}$, we only need $M_n$, $U_n$, and $\vx_{n+1}$.
Furthermore, $U_{n+1}$ is the desired interval robustness value over
the partial signal $\pvx{n+1}$.  Thus storing and iteratively updating
the two interval-values $U_n$ and $M_n$ is enough to monitor the given
formula.

\noindent \textbf{(3)} $\alw(\varphi \vee \ev \psi)$, where $\varphi
\equiv f(\vx)\!>\!0$, and $\psi \equiv g(\vx)\!>\!0$.  Observe the
following:
\begin{equation}
\label{eq:alwevone}
\begin{array}{ll}
\introb(\alw(\varphi \vee \ev \psi), \pvx{n+1},0) & 
    = \dmin_{i\in[0,n+1]} \dmax\left(p_i, \dmax_{j\in[i,n+1]} q_j\right)   \\
&   = \dmin_{i\in[0,n+1]} \dmax\left(p_i, \dmax_{j\in[i,n]} q_j, q_{n+1}\right) 
\end{array}
\end{equation}
\noindent Repeatedely applying the equivalence \eqref{eq:equivone}
to the outer $\min$ in \eqref{eq:alwevone} we get:
\begin{equation}
\dmax\left(q_{n+1}, \dmin_{i\in[0,n+1]} \dmax\left(p_i, \dmax_{j\in[i,n]}q_j\right)\right)
\end{equation}
\noindent The inner $\min$ simplifies to:
\begin{equation}
\dmax\left(q_{n+1}, \dmin\left(p_{n+1}, \underline{\dmin_{i\in[0,n]}\left(\dmax\left(p_i, \dmax_{j\in[i,n]} q_j\right)\right)}\right)\right)
\end{equation}
Let $T_n$ denote the underlined term; note that we do not require any
data at time $t_{n+1}$ to compute it. Using the recurrence $T_{n+1} =
\dmax\left(q_{n+1}, \dmin\left(p_{n+1}, T_n\right)\right)$, we can obtain
the desired interval robustness value. The memory required is that for
storing the one interval value $T_n$. A similar result can be established
for the dual formula $\ev(f(\vx)\!>\!0 \wedge \alw (g(\vx)\!>\!0))$.

\noindent \textbf{(4)} $\alw\ev(\varphi)$, where $\varphi \equiv
f(\vx)\!>\!0$. Observe the following:
\begin{equation}
\introb(\alw\ev(\varphi,\pvx{n+1},0) = \dmin_{i \in [0,n+1]} \dmax_{j \in [i,n+1]} p_j 
\end{equation}
Rewriting the outer $\min$ operator and the inner $\max$ more
explicitly, we get:
\begin{equation}
\dmin\left(\underline{\dmin_{i \in [0,n]} \dmax\left(\dmax_{j\in [i,n]} p_j, p_{n+1}\right)}, \quad p_{n+1}\right) 
\end{equation}
Repeatedly using \eqref{eq:equivone} to simplify the above underlined term
we get:
\begin{equation}
\dmin\left(\dmax\left(p_{n+1}, \dmin_{i\in[0,n]} \dmax_{j\in[i,n]}
p_j\right), p_{n+1}\right)  = p_{n+1}.
\end{equation}

The simplification to $p_{n+1}$, follows from \eqref{eq:equivfour}.  Thus,
to monitor $\alw\ev(f(\vx)\!>\!0)$, we do not need to store any
information, as the interval robustness simply evaluates to that of the
predicate $f(\vx)\!>\!0$ at time $t_{n+1}$. A similar result can be
obtained for the dual formula $\ev \alw (f(\vx)\!>\!>0)$.

\noindent \textbf{(5)} $\ev(\varphi \wedge \ev (\psi))$, where
$\varphi \equiv f(\vx)\!>\!0$ $\psi \equiv \ev(g(\vx)\!>\!0))$.
Observe the following:
\begin{equation}
\label{eq:evev}
\introb(\ev( \varphi \wedge \ev(\psi)), \pvx{n+1}, 0) =
\dmax_{i\in[0,n+1]}\left(\dmin\left(p_i, \dmax_{j\in[i,n+1]} q_j\right)\right)
\end{equation}
\noindent We can rewrite the RHS of Eq.~\eqref{eq:evev} as the first
expression below. Applying the equivalence in \eqref{eq:equivtwo} and
\eqref{eq:equivthree} to the expression on the left, we get the expression on
the right.
\begin{equation}
\label{eq:evevone}
\begin{array}{ll}
\dmax\left(
\begin{array}{l}
\min\left( p_0, \max\left(q_0, \ldots, q_{n+1}\right) \right) \\
\cdots\\
\min\left( p_n, \max\left(q_n, q_{n+1}\right) \right) \\
\min\left( p_{n+1}, q_{n+1} \right) \\
\end{array}
\right) & = 
\dmax\left(
\begin{array}{l}
\min(p_0,q_0), \ldots, \min(p_0,q_{n+1}), \\
\cdots \\
\min(p_n,q_n), \min(p_n, q_{n+1}), \\
\min( p_{n+1}, q_{n+1} )
\end{array}
\right)
\end{array}
\end{equation}
Grouping terms containing $q_{n+1}$ together and applying the equivalence
in \eqref{eq:equivtwo} we get:
\begin{equation}
\max\left(
\begin{array}{l}
\max\left(
\begin{array}{l}
\min(p_0,q_0), \min(p_0,q_1), \ldots, \min(p_0,q_n), \\
\min(p_1,q_1), \ldots, \min(p_1,q_n), \\
\cdots \\
\min(p_n,q_n)
\end{array}
\right), \\
\min(q_{n+1}, \underline{\max(p_0,p_1,\ldots,p_n)}),\\
\min(p_{n+1}, q_{n+1})
\end{array}
\right)
\end{equation}
\noindent Observe that the first argument to the outermost $\max$ can be
computed using only $\vx_1,\ldots,\vx_n$. Suppose we denote this term
$T_n$. Also note that in the second argument, the inner $\max$ (underlined)
can be computed using only $\vx_1,\ldots,\vx_n$. Let us denote this term by
$M_n$. We now have a recurrence relations:
\begin{eqnarray}
M_{n+1} & = & \max(M_n, p_{n+1}), \\
T_{n+1} & = & \max(T_n, \min(q_{n+1}, M_n), \min(q_{n+1}, p_{n+1})),
\end{eqnarray}
\noindent where $T_0$ = $\min(p_0,q_0)$ and $M_0$ = $p_0$. Thus, the
desired interval robustness can be computed using only two values stored in
$T_n$ and $M_n$. The dual result holds for the formula 
$\alw(\varphi \vee \alw (\psi))$.
\end{proof}

\noindent{\em Remarks on extending above result:}
The result in Theorem~\ref{thm:finiteness} can be generalized to allow
$\varphi$ and $\psi$ that are not atomic predicates, under following two
conditions:
\begin{enumerate}
\item
Bounded horizon subformulae condition: For each formula, the subformulae
$\varphi$ and $\psi$ have a bounded time-horizon, \ie, $\scope(\varphi)$
and $\scope(\psi)$ are closed intervals.
\item
Smallest step-size condition: Consecutive time-points in the signal
are at least $\Delta$ seconds apart, for some finite $\Delta$, which is
known {\em a priori}.
\end{enumerate}

We defer the proof of the general case to the full version of the paper
\cite{robust_monitoring_arxiv}, but remark that the proof techniques are
very similar. Let $\last$ denote the least upper bound of the time horizon
for all subformulae of a given untimed formula.  At any time $t_n$,
additional book-keeping is required to store partial information for
time-points in the range $[t_n - \last, t_n]$. By the step-size condition
there can be at most $\lceil \frac{\last}{\Delta} \rceil$ time-points in
this range.  This is then used to show that constant memory proportional to
$\lceil \frac{\last}{\Delta} \rceil$ is sufficient to monitor such an
untimed formula (with bounded-horizon subformulae).


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

